Knowledge Sharing via Domain Adaptation in Customs Fraud Detection

Knowledge of the changing traffic is critical in risk management. Customs offices worldwide have traditionally relied on local resources to accumulate knowledge and detect tax fraud. This naturally poses countries with weak infrastructure to become tax havens of potentially illicit trades. The current paper proposes DAS, a memory bank platform to facilitate knowledge sharing across multi-national customs administrations to support each other. We propose a domain adaptation method to share transferable knowledge of frauds as prototypes while safeguarding the local trade information. Data encompassing over 8 million import declarations have been used to test the feasibility of this new system, which shows that participating countries may benefit up to 2-11 times in fraud detection with the help of shared knowledge. We discuss implications for substantial tax revenue potential and strengthened policy against illicit trades.

==> 6_supplements.tex <==
\clearpage
\section{Supplementary Material}

\paragraph{Code Release.} 
Implementation of \ours{} is included in code supplementaries. We plan to publish an interactive tutorial that contains a series of procedures to compress knowledge, refine data using compressed knowledge, and perform fraud detection.


\paragraph{Data Details.} 
The format of import declarations varies slightly. We only consider the common fields, including numeric variables such as item price, weight, quantity, and categorical variables such as HS6 code, country code. The data also contained inspection results indicating whether each declaration was judged fraud or not, and the amount of tax raised after inspection. We 
report the raw variables of import declarations in Table~\ref{Tab:variable_description}. 

\begin{table}[h!]
\centering
\caption{Overview of the transaction-level import data, in which the description of each variable are provided.}
\scalebox{0.75}{
\begin{tabular}{l|l}
\toprule
Variable & Description  \\ \midrule


\textit{Quantity} & The specified number of items\\
\textit{Gross weight} & The physical weight of the items \\
\textit{HS code}   &  Applicable item code based on the harmonised system \\
\textit{Country code}  & Country from which the goods were imported \\
\textit{CIF value} & Transaction value including the insurance and freight costs \\ 
\textit{Total taxes} & Tariffs calculated by initial declaration \\ \midrule
\textit{Illicit ($y$)} & Target binary variable indicating whether the item is fraud \\
\textit{Revenue} & Amount of tax raised after the inspection, used for evaluation \\
\bottomrule 
\end{tabular}}
\label{Tab:variable_description}
\end{table}


\paragraph{Training Details.} 
For every country, the model $f$ is individually pre-trained for 10 epochs and fine-tuned for 30 epochs. The sharpening temperature $\tau$ in Eq~\eqref{eq:SCL_loss} was set as 0.07 by following previous works~\cite{gunel2020supervised}. Smaller SCL loss temperatures benefit training more than higher ones, but extremely low temperatures are harder to train due to numerical instability. The number of prototypes was set to 500 per class. We use the final month of each dataset as the test set, and the validation set was chosen as two weeks prior. The model was optimized using Ranger with a weight decay of 0.01~\cite{wright2021ranger21}. The batch size and learning rate were set as 128 and 0.005 for the entire training epochs. All models were run five times, and their average values were reported. 

\paragraph{Baseline Details.} 
Below are the detailed explanation of the baselines used in our experiments.
\begin{itemize}
\item Target Only: Measure the performance of a base fraud detection model $f(\cdot|\mathcal{D}_{t})$ trained on target data. The tree-based embedding model DATE is used~\cite{kim2020date} for $f$. DATE classifies and ranks illegal trade flows that contribute the
most to the overall customs revenue when caught.
\item Vanilla Transfer: Sharing parameters of the fraud detection model $f(\cdot|\mathcal{D}_{s})$ from source country $s$ and directly fine-tune using target dataset $\mathcal{D}_{t}$. 
\item Adaptive Transfer: Adaptive Knowledge Consistency (AKC) technique~\cite{abuduweili2021adaptive} is used to cope with the risk of negative transfer caused by the discrepancy between the source and target countries. It constrains the mean square error between the pre-trained feature extractor outputs and the target feature extractor outputs by adaptively sampling the target dataset $\mathcal{D}_{t}$. We perform a hard filter according to the sample importance by sorting fraud score difference between the source and target pre-trained models. The features with a lower 20 \% score difference were selected. 
\end{itemize}



\paragraph{Comprehensive Results.} 
Table~\ref{tab:results_all} shows the comprehensive results, which was simplified in Table~\ref{tab:singlesource} (Single-source scenarios) and Figure~\ref{fig:multisource} (Multi-source scenarios). From Table~\ref{tab:results_all}, we made Table~\ref{tab:singlesource} by picking single-source cases, and we drew Figure~\ref{fig:multisource} by averaging all multi-source \ours{} results grouped by the number of source countries.

Table~\ref{tab:results_label_increase} shows the original results, which was simplified in Figure~\ref{fig:target_size}. The table describes the performance gain by changing the target log size. From Table~\ref{tab:results_all}, we made Figure~\ref{fig:target_size} by averaging \ours{} results grouped by each target country. 

% Table~\ref{tab:results_all} also shows the full result of multi source performance evaluation. The pre-trained model of the source country showing the best performance in the validation set was used. The additional gain in raised tax is most noticeable for using a single source, yet there is a revenue gain with every added source. As the number of source countries increases, performance tends to increase by enriching the information. 


\paragraph{Dependency on Prototype Count.} 
Knowledge of frauds is shared as compressed representations called prototypes. The number of prototypes can determine the resolution of transferred knowledge. For instance, one may assume selective fraud patterns may be shared when limiting the prototype count. We test the sensitivity of the model on prototype count $|\mathcal{C}_s|$ by setting it from 10 to as large as the source data size $|\mathcal{D}_{s}|$. Table~\ref{tab:proto} shows detection performance remains intact by $|\mathcal{C}_s|$, implying that the model is not sensitive to the choice of hyper-parameters as long as the prototypes are used. 

% Data privacy can be increased by dramatically reducing the number of prototypes, \mc{=why?=}
% In addition, our memory-based approach can deliver source country information by only using prototypes without model hyper-parameters, unlike other frameworks. (See supplementary)

%In a nutshell, we can deliver source-enhanced information to the target while minimizing the leakage of source country information. 
% \newline \sd{저는 모델 parameter 안 넘겨주고 prototype만 넘겨줬을 때의 실험 결과도 서플리 말고 이 section에 같이 넣으면 좋겠어요. 모델 파라미터가 함께 전달될때는 프로토타입 개수에 따른 퍼포먼스가 크게 차이가 없다는 점을 확인했는데, 이 결과만으로는 그닥 이 섹션이 의미가 없는 거 같아요. 모델 파라미터가 전달되지 않을 때에는 프로토타입 개수랑 퍼포먼스 간에 상관관계가 있을 거 같아요.}

\begin{table}[h!]
\centering
\caption{Sensitivity analysis to the number of prototypes for country N. $|\mathcal{D}_{s}|$ implies that the entire embeddings are transferred instead of the clustered prototypes.}
\small
\scalebox{1}{
\begin{tabular}{c|ccccc}
\toprule
$|\mathcal{C}_s|$ & 0 & 10 & 100        & 1,000   &   $|\mathcal{D}_{s}|$ \\ \midrule
\textsf{M} $\rightarrow$ \textsf{N} & 0.6667  & 0.6714  & 0.6721  & 0.6681 & 0.6709\\
\textsf{C} $\rightarrow$ \textsf{N} & 0.6564 & 0.6656      & 0.6727 & 0.6863 & 0.6711\\
\textsf{T} $\rightarrow$ \textsf{N} & 0.6762 & 0.7379      & 0.7307 & 0.7286 & 0.7314\\
\bottomrule 
\end{tabular}
}
\label{tab:proto}
\end{table}


% \scalebox{0.85}{\begin{tabular}{c|ccccc}
% \toprule
% $|\mathcal{C}_s|$ & 0 & 10 & 100        & 1,000   &   $|\mathcal{D}_{s}|$ \\ \midrule
% M      & 0.6667 &0.6714  & 0.6721  & 0.6681 & 0.6709\\
% C         & 0.6564    &0.6656      & 0.6727 & 0.6863 & 0.6711\\
% T          &  0.6762   &0.7379      & 0.7307 & 0.7286 & 0.7314\\
% \bottomrule 
% \end{tabular}}
% \label{tab:proto}

% \scalebox{0.85}{\begin{tabular}{c|ccccc}
% \toprule
% $|\mathcal{C}_s|$ & 0 & 10 & 100        & 1,000   &   $|\mathcal{D}_{s}|$ \\ \midrule
% N      & 0.3051 &0.6714  & 0.6721  & 0.6681 & 0.6709\\
% C         & 0.6564    &0.6656      & 0.6727 & 0.6863 & 0.6711\\
% T          &  0.6762   &0.7379      & 0.7307 & 0.7286 & 0.7314\\
% \bottomrule 
% \end{tabular}}
% \label{tab:proto}



% Additional experiments: 리뷰어들이 어려운 걸 원하진 않을 거 같고 심플한 케이스들을 궁금해할 것 같음

% 추가할 만한 실험 1: Model parameter가 전달되지 않고 prototype만 전달하는 상황에서 성능 확인 & Table 3에 해당하는 prototype 개수 바꿔가며 성능 체크

% 추가할 만한 실험 2: Prototype을 만드는데 사용하는 source data를 현재는 전체 데이터의 n%로 두었는데, absolute하게 k개 (k=10000?)로 fix하고 돌리면 어떤 국가가 도움을 줄 것인가? 

% 추가할 만한 실험 3: 우리 예제의 경우 source country도 다 개발 도상국이고 DATE처럼 좋은 모델을 사용하지 않을 것임. 따라서 labeled data의 경우에도 그렇게 좋은 데이터가 아닐 텐데, 그저 그런 걸 공유하였을 때에도 도움이 되는가?  성원: target country의 corruption 



\input{tables/results_all.tex}
\input{tables/results_label_increase.tex}



% \subsection{Received comments}

% % Introduction - 현실화되려면 어려움이 있는데, 그 어려움이 무엇이 있고, 지금은 비슷한 지역에서 test를 했는데, continent이 달라도 효과가 있는 지 점검이 필요하다. 데이터를 전달하는 등에서 법적인 hurdle이 해결되어야 한다. 한국 - 베트남 두 나라 사이에 trade agreement들이 있고, bi-lateral하게 두 나라 사이에서는 sharing하는 factor들이 있는데, 그런 예시들을 써 주면 이런 게 불가능한 것만도 아니다. 양쪽으로 end-to-end 블록체인 policy commission - scale을 얘기하는 것을 얘기해도 좋다. 서로 format도 맞추고, 정보 교류가 되고 있다 라는 점을 넣어 주면 좋겠다. 170개 국이 다 참가하는 것은 아니고, 

% % 각자 build하고 학습하는 것보다 이게 더 쉽다? 어렵다? 이걸 쓰면 좀더 학습에 필요한 -- 


% % 리뷰어가 할 만한 질문: 어려운 게 아니라 완전 심플한 케이스들? source country도 다 개발 도상국이고 DATE처럼 좋은 모델을 사용하지 않을 텐데. 따라서 labeled data의 경우에도 그렇게 좋은 데이터가 아닐 텐데, 그저 그런 걸 공유하였을 때에도 도움이 되는가?

% % Source data의 비율로 (5%, 1%)가 아니라, absolute하게 1000개, 5000개로 fix하고 돌리면 어떤 국가가 도움을 줄 것인가?


% % 레퍼런스가 적은 것 같다. 지금보다는 15개 정도 많아도 좋다


% % Figure 2를 설명할 때 contrastive learning을 왜 꼭 써야 하는가에 대한 intuition이 부족하다. Figure 6이 조금 앞에 와도 된다.


% \medskip
% Table 2의 실험 결과를 좀더 이해하고 싶어함. 
% \begin{itemize}
% \item 국가별 결과를 본문에 다 나열하지 말고 average 해서 report하는 것이 더 나을려나?
% \item T 데이터가 가장 잘 사는 나라이기도 하면서 데이터 양이 많아서, 이를 source로 활용하였을 때 성능이 일반적으로 더 높아짐. M에 대해서만 성능 향상폭이 최고치는 아님
% \item 비슷한 국가를 source로 활용하였을 때 성능이 높아졌다는 점 어필 가능. 
% \item DATE의 input으로 source data를 같이 넣었을 때의 성능 증가 경향성이 DAS의 input으로 source data를 같이 넣었을 때의 성능 증가 경향성과 다르다: 이유가 무엇? DATE의 input으로 source와 target 데이터를 함께 넣었을 때는 negative transfer 등의 부작용이 발생하나? T 데이터를 함께 썼을 때 성능 증가가 오히려 적었다.
% \end{itemize}

% \medskip
% 동현: Transfer learning으로 인한 성능 향상이 다 높으면 상관없는데, 그다지 좋지 않은 경우가 발생했을 때 설명하기 위해서는 신빙성 있는 근거가 좀더 필요하고, 이에 대한 분석이 좀 필요함. Negative transfer가 발생했다 라고만 말하면 신빙성이 부족함, 예를 들면 GDP가 다르고 이로 인해 \& 무역 패턴이 어떠어떠한 이유로 다르다는 점을 데이터를 통해 알 수 있다 정도의 레벨로 얘기하면 좋겠음. 

% \medskip
% \ours{}는 Source 국가의 prototype과 모델 파라미터를 전달해 주는데, 더 간단한 방법은 무엇이 있는가? 이 관점에서 비교할 만한 baseline들이 더 필요하지 않을까? 

% \begin{itemize}
% \item 간단한 baseline (교수님): Source 국가의 우범에서 자주 등장하는 top-k HS 코드나 country code 등 간단한 정보만을 target 국가에 알려 주는 방법?
% \item Prototype만 주는 경우
% \item Model parameter만 주는 경우
% \end{itemize}




% \medskip

% Security concern: Source country의 model parameters와 prototype을 전달해 주는데, 이 정보를 이용해도 source data의 reidentification이 불가능하다는 점을 보여주면 좋겠음. Safety 관점에서의 수치를 보여주면 좋겠다?


% \medskip

% 교수님이 생각하는 우리 방법의 장점?
% \begin{itemize}
% \item Data의 representation 자체가 나가지 않음
% \item Importer 정보 등 민감성 정보가 나갈 일 없음
% \item Source data의 labeled data (우범성 정보)를 위주로 prototype을 만들기 때문에, original dataset의 distribution을 파악할 수 없음. 주는 정보와 안 주는 정보의 차이가 크기 때문에 괜찮음
% \end{itemize}








% duplicated contents are removed.

% Due to space limitation, we report the simplified result in main script. The actual figures are summarized in Table~\ref{tab:results_all}--\ref{tab:results_label_increase}.
% on all combinations of the source and target pairs in our main setup, which the source country shares knowledge based on the 5\% of its fraud-like logs and a target dataset has 1\% of randomly labeled logs. 

% This knowledge is used in four different ways: (1) no sharing at all, (2) standard fine-tuning by sharing model parameters of $f(\cdot|\mathcal{D}_{s})$ directly with the target country, (3) transfer learning based on the adaptive knowledge consistency technique~\cite{abuduweili2021adaptive},
%to alleviate the negative transfer problem caused by discrepancy between the source and the target data =do we need to say this?=}, % and (4) the proposed prototype-based memory bank.
% At the receiving end, we assume the target country has a weaker infrastructure and utilize only 1\% of trades for training. This assumption is simulated by randomly masking the log labels. 











==> 7_rebuttal.tex <==
\section{Author Response}

We appreciate all the reviewers' thoughtful feedback that improves our work. Please find our responses below.

\section{Response to Reviewer 1}
\subsubsection{Q1. \textit{Difficulty to create similar datasets for other countries.}}\mbox{}
Import declaration data is readily available by customs administrations of any country. Currently, 183 member countries of the World Customs Organizations are responsible for customs controls representing more than 98\% of all international trade. These countries utilize compatible clearance systems to handle import declarations such as ASYCUDA, UNIPASS, TradeNet, etc. The data format of these systems is similar by nature, as import declaration data need to be handled by parties in two countries.

\subsubsection{Q2. \textit{Manual effort to generate the data set.}}\mbox{} 
Custom officers determine Frauds during physical inspections, and the AI-based fraud detection model can recommend which items to check with priority to ease this process. For countries where an algorithmic fraud detection system is absent or weak, a lot of time and effort is required to inspect each transaction. In fact countries reported a total inspection was not feasible during COVID-19. The purpose of our study is to reduce such human effort through domain adaptation. 

\subsubsection{Q3. \textit{Can such data be constructed from multi-lingual data?}}\mbox{} We consider the most common fields in import declarations (i.e., product category, price, quantity, weight) to make it easily applicable in various regions. The current model does not utilize product descriptions from data providers, but they can be used as additional information to boost the performance of a selection model. Product descriptions written in various languages can be handled by a text encoder such as multilingual BERT. We are thankful for this suggestion, and we will consider this idea in the future.





\section{Response to Reviewer 2}
\subsubsection{Q1. \textit{The key problem will be deployment, and acceptance of this system.}}\mbox{} Thank you for sharing this practical concern, which we also agree. Our work was initiated by the increasing need to utilize machine learning in fraud detection shared by participating member countries of the World Customs Organizations. One of the concerns was the lack of infrastructure in developing countries to manage the system and adapt to changing traffic continually. A centrally managed memory bank system that we explored is one such possibility. As more countries are setting up bilateral agreements to share logs, we envision our model can facilitate such data sharing in the near future. 





\section{Response to Reviewer 3}


\subsubsection{Q1. \textit{Concerns regarding the re-identification from the memory bank.}}\mbox{}
We would be happy to add some more details to the data description. We agree there could be more evaluation on the re-identification prospect, which can develop as a separate piece of work. 
%
To our understanding, it is nearly impossible to re-identify information from a memory bank because the prototype generation process can be regarded as a ``hash-like" approach (where the input is hashed and become a scrambled representation of itself). To re-identify any information, adversarial actors should utilize brute-force-based or rainbow memory attacks, which are computationally expensive. We hence considered passing the embedding representation through a memory bank to be much safer than sharing the raw data. We also note that many companies release their proprietary images and metadata to the public for data mining competitions through its embeddings. 

In customs relations, more countries are forming bilateral agreements to exchange specific information to help identify high-risk items before they arrive in their respective territories. Our work also utilizes shared information across customs offices. Thank you for your concern and suggestion. \looseness=-1

% of Imagenet pretrained networks instead of releasing their raw data sets.

% Under the black or grey box attack situation, adversarial actors should utilize brute-force based approach or rainbow memory attack to reconstruct data, which is practically impossible because of its computational cost. 


\subsubsection{Q2. \textit{Are transactions comparable across different countries legal frameworks? To me it seems that the difference in legality of certain products could harm the generalization of the approach.}}\mbox{} 
Customs offices in different countries employ a data format that is similar by nature, as import declaration data need to be handled by parties in two countries. Hence our model can be applied to most countries directly without the worry of compatibility issues. 

The reviewer is correct to point out that prohibited and restricted items may vary from country to country. Screening for some of these important goals can happen at a different stage of the inspection if not all handled by the refining stage of the shared prototypes. 
%but from the utilitarian point of view, we observed a significant performance improvement when the embeddings of the target country is refined with shared prototypes.
Nonetheless, please note that our model targets more common forms of fraud detection types related to undervaluation or misclassification that is internationally agreed upon, such as a mismatch in the product category, price, weight, and quantity. This problem scope is the same as other related research on customs fraud detection, such as DATE. We will clarify this problem scope in the camera ready version, thank you. 


\section{Response to Reviewer 4}
\subsubsection{Q1. \textit{This works contains few methodological improvement.}}\mbox{} Thank you for the clarification question. This research aimed to introduce a problem of adapting to changes in traffic from the context of customs fraud detection---a topic that is less explored yet has a huge potential impact for many developing countries. We proposed a memory-bank system with contrastive learning and utilized real data to demonstrate the feasibility of this system.

\subsubsection{Q2. \textit{Is there any defect of the current model? I would be happy to see that the authors do some analysis on failure cases, and provide some future works on model design.}}\mbox{} 
We would be happy to follow up on this suggestion and discuss the potential gain from alternative encoding and clustering methods. 
Our data show that the model performance does not improve substantially for unseen transactions. For example, a source country with few automobile transactions will not see much performance improvement in this category. Several closed set domain adaptation research also reported this weakness. We can adapt the open set domain adaptation method as future work to mitigate the categorical mismatch between datasets. \looseness=-1


==> algorithms/algo3.tex <==
\begin{algorithm}[bth]
\SetNoFillComment
\begin{flushleft}
 \textbf{Input:} Training set $X_t$, items received $\mathcal{B}_t$, inspection rate $r_t$\\
 \textbf{Output:} A batch of selected items $\mathcal{B}_t^S$ \\
 \SetAlgoLined
 \tcc{Corresponds to the selection part in Alg.~\ref{alg:active_custom_select}.}
 Train the \dat{} model using training set $X_t$;\\
 Get the \textsf{Rev@n\%} from validation set;\\
 \eIf{\textsf{Rev@n\%} > $\theta$}{
     Perform prediction on $\mathcal{B}_t$, get the predicted annotation $(\textbf{x}_i, \hat{y}_i^{cls}, \hat{y}_i^{rev})$ for each item $\textbf{x}_i \in \mathcal{B}_t$;\\
     Calculate the gradient embedding $g_{x_{i}}$ (Eq. \ref{eqn:embedding});\\
     Obtain the set $\mathcal{B}^S_t$ of $r_t|\mathcal{B}_t|$ items by $k$-means++ initialization;\\
 }{
     Obtain the set $\mathcal{B}^S_t$ of $r_t|\mathcal{B}_t|$ items by random sampling;\\
 }
 \caption{Dummy algorithm template to fill}
 \label{alg:exploration_strategy}
\end{flushleft}
\end{algorithm}

==> pgfplots/target_size.tex <==
\begin{figure}[h!]
    \centering
    \begin{subfigure}[b]{0.49\columnwidth}
        \captionsetup{width=\linewidth}
        \scalebox{0.49}{
        \begin{tikzpicture}
          \begin{axis}[
            % title  = Country M,
            xbar,
            reverse legend,
            y axis line style = { opacity = 0 },
            axis x line       = none,
            tickwidth         = 0pt,
            ytick             = data,
            xlabel= Revenue@5\%,
            ylabel= Target size,
            enlarge y limits  = 0.2,
            enlarge x limits  = 0.02,
            xmin = 0,
            xmax = 1,
            xticklabel style={
              /pgf/number format/precision=3,
              /pgf/number format/fixed},
            symbolic y coords = {10\%, 5\%, 2\%, 1\%},
            nodes near coords, 
            nodes near coords style = {
              /pgf/number format/fixed},
            legend style={at={(1.1,1)},anchor=north east}
          ]
          \addplot coordinates { (0.4463,1\%)         (0.6107,2\%)
                               (0.8108,5\%)  (0.9092,10\%) };
          \addplot coordinates { (0.0466,1\%)         (0.1488,2\%)
                                 (0.2799,5\%)  (0.8764,10\%) };
        
          \legend{Source enhanced, Target only}
          \end{axis}
        \end{tikzpicture}}
        \caption{Country M}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\columnwidth}
        \captionsetup{width=\linewidth}
        \scalebox{0.49}{
        \begin{tikzpicture}
          \begin{axis}[
            % title  = Country C,
            xbar,
            reverse legend,
            y axis line style = { opacity = 0 },
            axis x line       = none,
            tickwidth         = 0pt,
            ytick             = data,
            xlabel= Revenue@5\%,
            ylabel= Target size,
            enlarge y limits  = 0.2,
            enlarge x limits  = 0.02,
            xmin = 0,
            xmax = 0.4,
            xticklabel style={
              /pgf/number format/precision=3,
              /pgf/number format/fixed},
            symbolic y coords = {10\%, 5\%, 2\%, 1\%},
            nodes near coords,
            nodes near coords style = {
              /pgf/number format/fixed},
            legend style={at={(1.1,1)},anchor=north east}
          ]
          \addplot coordinates { (0.1993,1\%)         (0.2279,2\%)
                               (0.2688,5\%)  (0.2805,10\%) };
          \addplot coordinates { (0.0853,1\%)         (0.2013,2\%)
                                 (0.2166,5\%)  (0.2614,10\%) };
          \end{axis}
        \end{tikzpicture}}
        \caption{Country C}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\columnwidth}
        \captionsetup{width=\linewidth}
        \scalebox{0.49}{
        \begin{tikzpicture}
          \begin{axis}[
            % title  = Country N,
            xbar,
            reverse legend,
            y axis line style = { opacity = 0 },
            axis x line       = none,
            tickwidth         = 0pt,
            ytick             = data,
            xlabel= Revenue@5\%,
            ylabel= Target size,
            enlarge y limits  = 0.2,
            enlarge x limits  = 0.02,
            xmin = 0,
            xmax = 1,
            xticklabel style={
              /pgf/number format/precision=3,
              /pgf/number format/fixed},
            symbolic y coords = {10\%, 5\%, 2\%, 1\%},
            nodes near coords,
            nodes near coords style = {
              /pgf/number format/fixed},
            legend style={at={(1.1,1)},anchor=north east}
          ]
          \addplot coordinates { (0.6933,1\%)         (0.7576,2\%)
                               (0.8309,5\%)  (0.8530,10\%) };
          \addplot coordinates { (0.1837,1\%)         (0.1894,2\%)
                                 (0.8092,5\%)  (0.8428,10\%) };
          \end{axis}
        \end{tikzpicture}}
        \caption{Country N}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\columnwidth}
        \captionsetup{width=\linewidth}
        \scalebox{0.49}{
        \begin{tikzpicture}
          \begin{axis}[
            % title  = Country T,
            xbar,
            reverse legend,
            y axis line style = { opacity = 0 },
            axis x line       = none,
            tickwidth         = 0pt,
            ytick             = data,
            xlabel= Revenue@5\%,
            ylabel= Target size,
            enlarge y limits  = 0.2,
            enlarge x limits  = 0.02,
            xmin = 0,
            xmax = 0.4,
            xticklabel style={
              /pgf/number format/precision=3,
              /pgf/number format/fixed},
            symbolic y coords = {10\%, 5\%, 2\%, 1\%},
            nodes near coords,
            nodes near coords style = {
              /pgf/number format/fixed},
            legend style={at={(1.1,1)},anchor=north east}
          ]
          \addplot coordinates { (0.3179,1\%)         (0.3225,2\%)
                               (0.3348,5\%)  (0.3430,10\%) };
          \addplot coordinates { (0.1541,1\%)         (0.3076,2\%)
                                 (0.3260,5\%)  (0.3391,10\%) };
          \end{axis}
        \end{tikzpicture}}
        \caption{Country T}
    \end{subfigure}
\caption{Rev@5\% difference between base model and \ours{} by increasing target size. \ours{} brings a big performance improvement until there is enough data in the target country. \sd{=Another version of Figure 4, 어떤 그림이 더 좋을까요, 혹은 improvement된 비율만 보여줄까요? 어쩌면 표로 나타내도 될 거 같아요. 그려놓고 보니 Figure 4가 더 나은 거 같기도 한데. Figure 4를 좀더 예쁘게 바꿔볼까요? =}}
\label{fig:target_size}
\end{figure}

==> tables/deprecated/results_target_c.tex <==
\begin{table}[h!]
\centering
% \scriptsize
\caption{Customs selection performance in Country C boosted significantly by using additional countries datasets and domain adaptation technique.}
\label{tab:datastats}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{p{2cm} p{1.3cm} p{1.3cm} p{1.3cm} p{1.3cm}} \toprule
    Source and target ($c_s \rightarrow c_t$) & DATE \newline ($c_t$ only) & DATE \newline ($c_s + c_t$) & Other SOTA \newline ($c_s + c_t$) & Domain \newline Adaptation \newline ($c_s + c_t$)  \\ \midrule
    \textsf{M} $\rightarrow$ \textsf{C} & & & & \\
    \textsf{N} $\rightarrow$ \textsf{C} & & & & \\
    \textsf{T} $\rightarrow$ \textsf{C} & & & & \\
    \textsf{M}$+$\textsf{N} $\rightarrow$ \textsf{C} & & & & \\
    \textsf{M}$+$\textsf{T} $\rightarrow$ \textsf{C} & & & & \\
    \textsf{N}$+$\textsf{T} $\rightarrow$ \textsf{C} & & & & \\
    \textsf{M}$+$\textsf{N}$+$\textsf{T} $\rightarrow$ \textsf{C} & & & & \\
    \bottomrule
\end{tabular}
% }
\end{table}

==> tables/deprecated/results_target_m.tex <==
\begin{table}[h!]
\centering
% \scriptsize
\caption{Customs selection performance in Country M boosted significantly by using additional countries datasets and domain adaptation technique.}
\label{tab:datastats}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{p{2cm} p{1.3cm} p{1.3cm} p{1.3cm} p{1.3cm}} \toprule
    Source and target ($c_s \rightarrow c_t$) & DATE \newline ($c_t$ only) & DATE \newline ($c_s + c_t$) & Other SOTA \newline ($c_s + c_t$) & Domain \newline Adaptation \newline ($c_s + c_t$)  \\ \midrule
    \textsf{N} $\rightarrow$ \textsf{M} & 0.0581 & 0.5055 & & 0.6320 \\
    \textsf{C} $\rightarrow$ \textsf{M} & & & & \\
    \textsf{T} $\rightarrow$ \textsf{M} & & & & \\
    \textsf{N}$+$\textsf{T} $\rightarrow$ \textsf{M} & & & & \\
    \textsf{N}$+$\textsf{C} $\rightarrow$ \textsf{M} & & & & \\
    \textsf{C}$+$\textsf{T} $\rightarrow$ \textsf{M} & & & & \\
    \textsf{N}$+$\textsf{C}$+$\textsf{T} $\rightarrow$ \textsf{M} & & & & \\ \bottomrule
\end{tabular}
% }
\end{table}

==> tables/deprecated/results_target_n.tex <==
\begin{table}[h!]
\centering
% \scriptsize
\caption{Customs selection performance in Country M boosted significantly by using additional countries datasets and domain adaptation technique.}
\label{tab:datastats}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{p{2cm} p{1.3cm} p{1.3cm} p{1.3cm} p{1.3cm}} \toprule
    Source and target ($c_s \rightarrow c_t$) & DATE \newline ($c_t$ only) & DATE \newline ($c_s + c_t$) & Other SOTA \newline ($c_s + c_t$) & Domain \newline Adaptation \newline ($c_s + c_t$)  \\ \midrule
    \textsf{M} $\rightarrow$ \textsf{N} & & & & \\
    \textsf{C} $\rightarrow$ \textsf{N} & & & & \\
    \textsf{T} $\rightarrow$ \textsf{N} & & & & \\
    \textsf{M}$+$\textsf{C} $\rightarrow$ \textsf{N} & & & & \\
    \textsf{M}$+$\textsf{C} $\rightarrow$ \textsf{N} & & & & \\
    \textsf{M}$+$\textsf{C} $\rightarrow$ \textsf{N} & & & & \\
    \textsf{M}$+$\textsf{C}$+$\textsf{T} $\rightarrow$ \textsf{N} & & & & \\
    \bottomrule
\end{tabular}
% }
\end{table}

==> tables/results_all.tex <==
\begin{table*}[t!]
\centering
% \scriptsize
\caption{Full results on both single- and multi-source case.}
\label{tab:results_all}
% \resizebox{\pagewidth}{!}{%
\begin{tabular}{l|cccc} \toprule
    Test & Target & Vanilla & Adaptive  &  Proposed \\
    Setup & Only & Transfer & Transfer &  \ours{} \\ \midrule
    \textsf{N} $\rightarrow$ \textsf{M} & 0.0466 $\pm$ 0.0075 & 0.0681 $\pm$ 0.0007 &  0.1091 $\pm$ 0.0039 & 0.5152 $\pm$ 0.0066 \\
    \textsf{C} $\rightarrow$ \textsf{M} & & 0.0869 $\pm$ 0.0010 & 0.1405 $\pm$ 0.0012 & 0.5271 $\pm$ 0.0074\\
    \textsf{T} $\rightarrow$ \textsf{M} &  & 0.2112 $\pm$ 0.0041 & 0.2458 $\pm$ 0.0027 & 0.2966 $\pm$ 0.0237\\
    \textsf{N}$+$\textsf{T} $\rightarrow$ \textsf{M} & & & & 0.5107 $\pm$ 0.0049\\
    \textsf{N}$+$\textsf{C} $\rightarrow$ \textsf{M} & & & & 0.5385 $\pm$ 0.0136\\
    \textsf{C}$+$\textsf{T} $\rightarrow$ \textsf{M} & & & & 0.5426 $\pm$ 0.0114\\
    \textsf{N}$+$\textsf{C}$+$\textsf{T} $\rightarrow$ \textsf{M} & & & & 0.5435 $\pm$ 0.0095\\
    \midrule
    \textsf{M} $\rightarrow$ \textsf{C}   & 0.0853 $\pm$ 0.0042 & 0.1806 $\pm$ 0.0026 & 0.1843 $\pm$ 0.0011 & 0.1915 $\pm$ 0.0066\\
    \textsf{N} $\rightarrow$ \textsf{C} & & 0.0297 $\pm$ 0.0028 & 0.1081 $\pm$ 0.0009 & 0.1794 $\pm$ 0.0065\\
    \textsf{T} $\rightarrow$ \textsf{C} & & 0.0719 $\pm$ 0.0014 & 0.1402 $\pm$ 0.0043 &  0.2271 $\pm$ 0.0015\\
    \textsf{M}$+$\textsf{N} $\rightarrow$ \textsf{C} & & & & 0.2154 $\pm$ 0.0045\\
    \textsf{M}$+$\textsf{T} $\rightarrow$ \textsf{C} & & & & 0.2339  $\pm$ 0.0061\\
    \textsf{N}$+$\textsf{T} $\rightarrow$ \textsf{C} & & & & 0.2328 $\pm$  0.0053\\
    \textsf{M}$+$\textsf{N}$+$\textsf{T} $\rightarrow$ \textsf{C} & & & & 0.2340  $\pm$ 0.0042\\  
    \midrule
    \textsf{M} $\rightarrow$ \textsf{N} & 0.1837 $\pm$ 0.0063 & 0.1018  $\pm$  0.0024 & 0.3244 $\pm$ 0.0099 & 0.6681 $\pm$ 0.0159\\
    \textsf{C} $\rightarrow$ \textsf{N} & & 0.2368  $\pm$ 0.0122 & 0.4043 $\pm$ 0.0023 & 0.6863 $\pm$ 0.0097 \\
    \textsf{T} $\rightarrow$ \textsf{N} & &  0.1119 $\pm$ 0.0031 & 0.3032 $\pm$ 0.0295 & 0.7286 $\pm$ 0.0093\\
    \textsf{M}$+$\textsf{C} $\rightarrow$ \textsf{N} & & & & 0.6887 $\pm$  0.0127\\
    \textsf{M}$+$\textsf{T} $\rightarrow$ \textsf{N} & & & & 0.7387 $\pm$ 0.0033\\
    \textsf{T}$+$\textsf{C} $\rightarrow$ \textsf{N} & & & & 0.7347 $\pm$  0.0020\\
    \textsf{M}$+$\textsf{C}$+$\textsf{T} $\rightarrow$ \textsf{N} & & & & 0.7395 $\pm$ 0.0051\\ 
    \midrule
    \textsf{M} $\rightarrow$ \textsf{T} & 0.1541 $\pm$ 0.0348 & 0.3005 $\pm$ 0.0021 & 0.3037 $\pm$ 0.0009 & 0.3181 $\pm$ 0.0068 \\
    \textsf{C} $\rightarrow$ \textsf{T} & & 0.2844 $\pm$ 0.0015 & 0.3012 $\pm$ 0.0013 & 0.3073 $\pm$ 0.0007\\
    \textsf{N} $\rightarrow$ \textsf{T} & & 0.2007 $\pm$ 0.0023 & 0.3033 $\pm$ 0.0007 & 0.3282 $\pm$  0.0034\\
    \textsf{M}$+$\textsf{C} $\rightarrow$ \textsf{T} & & & & 0.3161 $\pm$ 0.0024\\
    \textsf{M}$+$\textsf{N} $\rightarrow$ \textsf{T} & & & & 0.3292 $\pm$ 0.0021\\
    \textsf{C}$+$\textsf{N} $\rightarrow$ \textsf{T} & & & & 0.3291 $\pm$ 0.0030\\
    \textsf{M}$+$\textsf{C}$+$\textsf{N} $\rightarrow$ \textsf{T} & & & & 0.3286 $\pm$ 0.0017\\ 
    \bottomrule
    
    % }
\end{tabular}
\end{table*}


\if 0
\begin{table*}[t!]
\centering
% \scriptsize
\caption{Full results  Revenue@5% performance und in both single- and multi- source.  \sd{5\%에 돌린 실험 결과도 여기에도 일단 채워 넣어 둬요.}}
% (상세 실험 세팅: 지원국의 경우, 전체 데이터의 5\%만 검사된 세팅을 가정하였다. 보다 상세하게는, 초기 일부 데이터 (5\%)를 활용하여 DATE 모델을 학습, 나머지 데이터 중 가장 우범도가 높은 5\%만 검사되었다고 생각하고 라벨을 남겨놓음, 나머지 95\%의 경우 라벨을 제거함, domain adaption을 위해서 검사가 된 5\% 데이터를 도입국에 지원. 도입국의 경우, 마지막 1년을 hold out 테스트 셋으로 삼고, 이전 1년 데이터를 학습 데이터로 삼음. 모델이 갖춰지지 않았다는 점을 고려하여, 학습 데이터 중 랜덤하게 5\%만 라벨이 있다고 세팅. 나머지 데이터는 라벨을 제거하였음.)}
\label{tab:results_all}
% \resizebox{\pagewidth}{!}{%
\begin{tabular}{p{2.3cm}| p{1.3cm} p{1.3cm} p{1.3cm} p{1.3cm} | p{1.3cm} p{1.3cm} p{1.3cm} p{1.3cm}} \toprule
     & \multicolumn{4}{c|}{Target data used = 1\%} & \multicolumn{4}{c}{5\%} \\ \cmidrule{2-9}
    Source country \newline to target country \newline ($c_s \rightarrow c_t$) & DATE \newline ($c_t$ only) & DATE \newline ($c_s + c_t$) & AKC \newline ($c_s + c_t$) & \ours{} ($c_s + c_t$) & DATE \newline ($c_t$ only) & DATE \newline ($c_s + c_t$) & AKC \newline ($c_s + c_t$) & \ours{} ($c_s + c_t$)  \\
    \midrule
    \textsf{N} $\rightarrow$ \textsf{M} & 0.0466 & 0.0681& & 0.5152 & & & & \\
    \textsf{C} $\rightarrow$ \textsf{M} & & 0.0869 & & 0.5271 & & & & \\
    \textsf{T} $\rightarrow$ \textsf{M} &  & 0.2112 & & 0.2966 & & & & \\
    \textsf{N}$+$\textsf{T} $\rightarrow$ \textsf{M} & & & & 0.5107 & & & & \\
    \textsf{N}$+$\textsf{C} $\rightarrow$ \textsf{M} & & & & 0.5385 & & & & \\
    \textsf{C}$+$\textsf{T} $\rightarrow$ \textsf{M} & & & & 0.5426 & & & & \\
    \textsf{N}$+$\textsf{C}$+$\textsf{T} $\rightarrow$ \textsf{M} & & & & 0.5435\\
    \midrule
    \textsf{M} $\rightarrow$ \textsf{C} & 0.0853 & 0.1806  &  & 0.1915 & & & & \\
    \textsf{N} $\rightarrow$ \textsf{C} & & 0.0297 & & 0.1794 & & & & \\
    \textsf{T} $\rightarrow$ \textsf{C} & & 0.0719 & &  0.2271 & & & & \\
    \textsf{M}$+$\textsf{N} $\rightarrow$ \textsf{C} & & & & 0.2154 & & & & \\
    \textsf{M}$+$\textsf{T} $\rightarrow$ \textsf{C} & & & & 0.2339 & & & & \\
    \textsf{N}$+$\textsf{T} $\rightarrow$ \textsf{C} & & & & 0.2328 & & & & \\
    \textsf{M}$+$\textsf{N}$+$\textsf{T} $\rightarrow$ \textsf{C} & & & & 0.2340 \\  
    \midrule
    \textsf{M} $\rightarrow$ \textsf{N} & 0.1837 & 0.1018 & & 0.6651 & & & & \\
    \textsf{C} $\rightarrow$ \textsf{N} & & 0.2368 & & 0.6863 & & & & \\
    \textsf{T} $\rightarrow$ \textsf{N} & &  0.1119 & & 0.7286 & & & & \\
    \textsf{M}$+$\textsf{C} $\rightarrow$ \textsf{N} & & & & 0.6887 & & & & \\
    \textsf{M}$+$\textsf{T} $\rightarrow$ \textsf{N} & & & & 0.7387 & & & & \\
    \textsf{T}$+$\textsf{C} $\rightarrow$ \textsf{N} & & & & 0.7347 & & & & \\
    \textsf{M}$+$\textsf{C}$+$\textsf{T} $\rightarrow$ \textsf{N} & & & & 0.7395 \\ 
    \midrule
    \textsf{M} $\rightarrow$ \textsf{T} & 0.1541 & 0.3005 & & 0.3181 & & & & \\
    \textsf{C} $\rightarrow$ \textsf{T} & & 0.2844  & & 0.3073 & & & & \\
    \textsf{N} $\rightarrow$ \textsf{T} & & 0.2007 &  & 0.3282 & & & & \\
    \textsf{M}$+$\textsf{C} $\rightarrow$ \textsf{T} & & & & 0.3161 & & & & \\
    \textsf{M}$+$\textsf{N} $\rightarrow$ \textsf{T} & & & & 0.3292 & & & & \\
    \textsf{C}$+$\textsf{N} $\rightarrow$ \textsf{T} & & & & 0.3291 & & & & \\
    \textsf{M}$+$\textsf{C}$+$\textsf{N} $\rightarrow$ \textsf{T} & & & & 0.3286 & & & & \\ 
    \bottomrule
\end{tabular}
% }
\end{table*}

\fi

==> tables/results_label_increase.tex <==
\begin{table*}[t!]
\centering
% \scriptsize
\caption{Knowledge from source country is helpful until some degree of dataset is collected at target country.}
\label{tab:results_label_increase}
\resizebox{\linewidth}{!}{%
\begin{tabular}{p{2.3cm} | c c | c c | c c | c c } \toprule & \multicolumn{2}{c|}{Target used = 1\%} & \multicolumn{2}{c|}{2\%} & \multicolumn{2}{c|}{5\%} & \multicolumn{2}{c}{10\%} \\ \cmidrule{2-9}

    Source country \newline to target country \newline ($c_s \rightarrow c_t$) & Target Only & \ours{}& Target Only & \ours{}& Target Only & \ours{} & Target Only & \ours{}  \\ \midrule
    \textsf{N} $\rightarrow$ \textsf{M} & 0.0466 & 0.5152 & 0.1488 & 0.6045 & 0.2799 & 0.8068 & 0.8764 & 0.9164 \\
    \textsf{C} $\rightarrow$ \textsf{M} & &  0.5271 & & 0.6915 &  & 0.8036 &  & 0.9085\\
    \textsf{T} $\rightarrow$ \textsf{M} & &  0.2966 & & 0.5360 & & 0.8220 & & 0.9028\\
    \midrule
    \textsf{M} $\rightarrow$ \textsf{C} & 0.0853 & 0.1915 & 0.2013 & 0.2113 & 0.2166 & 0.2697 & 0.2614 & 0.2971 \\
    \textsf{N} $\rightarrow$ \textsf{C} & & 0.1794 & & 0.2470 & & 0.2637 & & 0.2713 \\
    \textsf{T} $\rightarrow$ \textsf{C} & & 0.2271 & & 0.2255 & & 0.2731 & & 0.2730\\
    \midrule
    \textsf{M} $\rightarrow$ \textsf{N} & 0.1837 & 0.6651 & 0.1894 & 0.7632 & 0.8092 & 0.8285 & 0.8428 & 0.8697 \\
    \textsf{C} $\rightarrow$ \textsf{N} & &  0.6863 & & 0.7397 & & 0.8321 & & 0.8483\\
    \textsf{T} $\rightarrow$ \textsf{N} & & 0.7286 & & 0.7699 & & 0.8322 & & 0.8410\\
    \midrule
    \textsf{M} $\rightarrow$ \textsf{T} & 0.1541 & 0.3181 & 0.3076& 0.3172 & 0.3260 & 0.3332 & 0.3391 & 0.3439\\
    \textsf{C} $\rightarrow$ \textsf{T} & & 0.3073 & & 0.3246 & & 0.3376 & & 0.3410\\
    \textsf{N} $\rightarrow$ \textsf{T} & & 0.3282& & 0.3257 & & 0.3335 & & 0.3442\\
    \bottomrule
\end{tabular}
}
\end{table*}
